In Silico Study for Optimizing Intensity and Focality Electrode Configurations for Directional DBS Under Uncertainty Using Metaheuristic L1L1 Method

Background and Objective: As Deep Brain Stimulation (DBS) advances toward directional leads and optimization-based current steering, selecting electrode contact configurations becomes complex. This study formulates configuration selection as an inverse mapping between target activation and electrode currents using metaheuristic L1-norm regularized L1-norm fitting (L1L1). L1L1 incorporates lead-field uncertainty arising from electrode placement, tissue properties, and forward modeling assumptions. Methods: The framework introduces lead-field perturbations and restricts the controllable domain through a sensitivity-based feasibility criterion within a finite element formulation derived using the Complete Electrode Model. Current distributions were optimized for 8- and 40-contact leads. Performance was evaluated using focused current density, nuisance current density, and their ratio under safety and sparsity constraints. Results: L1L1 was evaluated using noiseless and noisy lead fields, with noise selected to reflect attenuation within the volume of tissue activated. The method produced sparse, spatially selective stimulation patterns across perturbation levels. Hyperparameter optimization yielded bipolar or multipolar configurations. Compared with the Reciprocity Principle (RP), which produced strictly bipolar configurations, and Tikhonov-regularized least squares (TLS), which produced more distributed solutions, L1L1 enabled controlled transitions between sparse and multipolar patterns. It concentrated stimulation within the target while limiting unintended current spread, particularly under noisy conditions. Conclusions: L1L1 can assist specialists in optimizing DBS configurations. By incorporating uncertainty directly into optimization, it provides robust and interpretable current steering across lead configurations while accounting for forward-model variability.

==> Figure_Norm_differences.tex <==
\begin{figure*}[ht!]
\centering
    \begin{footnotesize}
    \centering
    \fbox{
    \begin{minipage}{8.9cm}
        \centering
        8-contact electrode configuration \\
        %\includegraphics[height = 5.50cm, width = 0.50cm, angle = 90]{Figure_BoxPlot/AB_probe.png} \\
        \vskip0.2cm
        %%% A, B, C (Text)
        \begin{minipage}{0.35cm}
        \rotatebox{90}{Noiseless lead field}
        \end{minipage}
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType1_FOC.jpg} \\
            \textbf{A1.} {Focus} $\Gamma$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.7cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType1_NUS.jpg} \\
            \textbf{B1.} {Nuisance} $\Xi$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType1_RAT.jpg} \\
            \textbf{C1.} {Ratio} $\Theta$ (rel.)
        \end{minipage}
        %%%%
        \vskip0.2cm
        %%%% A, B, C
                \begin{minipage}{0.35cm}
        \rotatebox{90}{Noisy lead field}
        \end{minipage}
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType2_FOC.jpg} \\
            \textbf{G1.} {Focus} $\Gamma$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.7cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType2_NUS.jpg} \\
            \textbf{H1.} {Nuisance} $\Xi$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/AB_plot_LFType2_RAT.jpg} \\
            \textbf{I1.} {Ratio} $\Theta$ (rel.)
        \end{minipage}
        %%%% D, F, G
        %%%%
    \end{minipage}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{minipage}{8.9cm}
        \centering
        40-contact electrode configuration \\
        \vskip0.2cm
        %%% A, B, C (Text)
                \begin{minipage}{0.35cm}
        \rotatebox{90}{Noiseless lead field}
        \end{minipage}
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType1_FOC.jpg} \\
            \textbf{A2.} {Focus} $\Gamma$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.7cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType1_NUS.jpg} \\
            \textbf{B2.} {Nuisance} $\Xi$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType1_RAT.jpg} \\
            \textbf{C2.} {Ratio} $\Theta$ (rel.)
        \end{minipage}
        %%%%
        \vskip0.2cm
        %%%% D, E, F
        %%%% A, B, C
                \begin{minipage}{0.35cm}
        \rotatebox{90}{Noisy lead field}
        \end{minipage}
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType2_FOC.jpg} \\
            \textbf{G2.} {Focus} $\Gamma$ (A/m\textsuperscript{2})
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.7cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType2_NUS.jpg} \\
            \textbf{H2.} {Nuisance} $\Xi$ (A/m\textsuperscript{2}) \\
        \end{minipage}
        \hskip0.25cm
        \begin{minipage}{2.5cm}
            \centering
            \includegraphics[width = 2.50cm]{Figure_BoxPlot/plots/MED_plot_LFType2_RAT.jpg} \\
            \textbf{I2.} {Ratio} $\Theta$ (rel.) \\
        \end{minipage}
        \end{minipage}      }
               \begin{tikzpicture}
    \node[draw=none] at (0,0) {
        \begin{tabular}{llll}
                    \tikz \draw[blue, thick] (0,0) -- (0.6,0); & L1L1(A), $\varepsilon \in [-160, 0]$, Parallel &
            \tikz \draw[red, thick] (0,0) -- (0.6,0); & L1L1(B), $\varepsilon \in [-10, 0]$, Parallel \\
                        \tikz \draw[blue, dashed, thick] (0,0) -- (0.6,0); & L1L1(A), $\varepsilon \in [-160, 0]$, Perpendicular &
            \tikz \draw[red, dashed,thick] (0,0) -- (0.6,0); & L1L1(B), $\varepsilon \in [-10, 0]$, Perpendicular 
        \end{tabular}
    };
\end{tikzpicture} 
\end{footnotesize}
\caption{Performance of L1L1(A) and L1L1(B) for optimizing the field ratio $\Theta$ subject to criterion $\Gamma \geq \Gamma_0$ with noiseless and noisy (PSNR 40 dB) lead field. \textbf{Left:} (1) 8-contact, and \textbf{Right:} (2) 40-contact electrode configurations. L1L1(A) and L1L1(B)  suppress the nuisance current density $\Xi$ pattern using two different dynamic ranges, namely,  $\varepsilon \in [-160, 0]$ (blue) and $\varepsilon \in [-10,  0]$ (red), respectively. The results are sub-grouped by the direction of the current dipole, whether its alignment is parallel (solid line) or perpendicular (dotted line) with the applied lead. The degrees of freedom have been sorted according to ascending field ratio $\Theta$. The results show that the overly optimistic dynamic range applied in L1L1(A) results in very high field values of $\Theta$ in the noiseless case, which are, however, absent in the noisy one. In contrast, L1L1(B) is only marginally affected by the noise due to more realistic assumption of the maximum obtainable dynamic range under uncertainty. }
\label{Fig:Norm_differences_plot}
\end{figure*}

==> Figure_impedance.tex <==
\begin{figure}[h!]
    \centering
    \begin{minipage}[b]{0.235\textwidth}
        \centering
        \includegraphics[height=5.2cm]{Figure_impedance/leadfield_distribution.png}
    \end{minipage}
    \begin{minipage}[b]{0.235\textwidth}
        \centering
        \includegraphics[height=5.2cm]{Figure_impedance/leadfield_outliers.png}
    \end{minipage}
    \caption{\textcolor{black}{Comparison of lead field strength statistics for different probe configurations and impedance values. The results indicate that impedance-induced differences remain relatively minor compared to the mutual differences between the probe configurations themselves. In particular, increasing the contact count produces a substantially greater variation in lead field amplitude than the impedance variation across the feasible range. {\bf Left panel}: average lead field amplitude (mA/cm\textsuperscript{2}) for 8- and 40-contact probes evaluated for impedances set at 50~$\Omega$ and 2.0~k$\Omega$, representing the lower and upper extremes of the feasible impedance interval suggested in \cite{butson2006sources}. {\bf Right panel}: outlier distribution (mA/cm\textsuperscript{2}) beyond the 91st percentile, corresponding to the extent of the whiskers in the boxplot representation. The stacked bars separate the cumulative contribution of successive upper quantile intervals. As the larger impedance value of 2.0~k$\Omega$ systematically yields greater lead field amplitude and therefore, in theory, improved numerical optimization robustness, the 2.0~k$\Omega$ case was selected as the reference impedance throughout this study.}}
    \label{fig:leadfield_distribution_and_outliers} 
\end{figure}

==> tables/Table_Abbott.tex <==
\begin{table}[ht!]
\begin{normalsize}
\centering
\caption{Performance summary for the algorithm-optimized 8- and 40-contact probes. \textbf{{\em Bipolar}} configurations are obtained through the reciprocity principle while \textbf{{\em Multipolar}} through L1-norm fitting L1-norm Regularized (L1L1) method with the following indications: $\varepsilon = [-10, -160]$ dB (decibels); dipolar target current alignment either {\em Parallel} or {\em Perpendicular} with respect to the directional lead; numerical performance over a noiseless lead field and a SNR. Results are given for {\em Focused} ($\Gamma$) and {\em Nuisance} ($\Xi$) current densities, and {\em Field ratio} ($\Theta$).}
\renewcommand{\arraystretch}{1.25}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|r|rr|rr}
\multicolumn{2}{c|}{}           & \multicolumn{1}{c|}{\textbf{Bipolar}} & \multicolumn{2}{c|}{\textbf{-10dB}}                                        & \multicolumn{2}{c}{\textbf{-160dB}}                                       \\ \hline
\textbf{Values}           & \textbf{Vec} & \multicolumn{1}{c|}{\textbf{-}}       & \multicolumn{1}{c}{\textbf{Noiseless}} & \multicolumn{1}{c|}{\textbf{SNR}} & \multicolumn{1}{c}{\textbf{Noiseless}} & \multicolumn{1}{c}{\textbf{SNR}} \\ \hline
\multirow{2}{*}{Focused}  & \textit{1}   & 3.850                                 & 2.018                                  & \textit{2.236}                    & 2.195                                  & \textit{1.737}                   \\ \cline{3-7} 
                          & \textit{2}   & 3.850                                 & 3.369                                  & \textit{2.230}                    & 2.235                                  & \textit{2.287}                   \\ \hline
\multirow{2}{*}{Nuisance} & \textit{1}   & 0.741                                 & 0.107                                  & \textit{0.172}                    & 0.003                                  & \textit{0.203}                   \\ \cline{3-7} 
                          & \textit{2}   & 0.741                                 & 0.261                                  & \textit{0.199}                    & 0.003                                  & \textit{0.160}                   \\ \hline
\multirow{2}{*}{Ratio}    & \textit{1}   & 5.195                                 & 9.165                                  & \textit{8.491}                    & 526.440                                & \textit{7.564}                   \\ \cline{3-7} 
                          & \textit{2}   & 5.195                                 & 10.965                                 & \textit{8.469}                    & 536.050                                & \textit{9.959}                  
\end{tabular}%
}
\end{normalsize}
\label{Tab:Abbott}
\end{table}

==> tables/Table_Comparison_Methods_L1L1.tex <==
%\clearpage
\begin{table*}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.25}

\caption{
\textbf{Computational approaches for determining DBS stimulation parameters}. 
The optimization frameworks as follows derive electrode configurations or stimulation amplitudes are categorized depending on which stimulation settings are systematically evaluated. These are \emph{mathematical optimization frameworks}, solving an explicitly optimization problem defined on the electric-field or activation model \cite{pena2017pso_dbs,anderson2018dbs_programming,cubo2019dbs_optimization}; and \emph{model-guided and clinical programming frameworks}, using computational models, imaging-derived targets, or clinical-response measurements as fine-tuning references \cite{frankemolle2010computational_dbs,pourfar2015guide,heldman2016computer_guided_dbs,roediger2022stimfit,malekmohammadi2022illumina3d}. The proposed L1L1 method \cite{galaz2022l1l1} belongs to the first group, as it formulates stimulation design as an explicit optimization problem defined directly on the lead-field representation of the electric field.
}
\label{tab:dbs_methods_comparison}

\begin{tabular}{p{2.0cm} p{3.0cm} p{3.5cm} p{3.5cm} p{4.0cm}}
\hline
\textbf{Study} & \textbf{Optimization Variables} & \textbf{Method} & \textbf{Objective Function} & \textbf{Field / Activation Model} \\
\hline

\multicolumn{5}{l}{\textbf{Mathematical optimization frameworks}}\\
\hline

\cite{pena2017pso_dbs}
& Contact configuration, amplitudes
& Particle swarm optimization
& Pathway targeting
& Pathway activation from FEM fields \\

\cite{anderson2018dbs_programming}
& Contact currents
& Nonlinear optimization
& Target activation / avoidance suppression
& Hessian-based activation surrogate \\

\cite{cubo2019dbs_optimization}
& Contact amplitudes
& Constrained optimization
& Maximize target VTA
& VTA threshold model \\

\cite{galaz2022l1l1}
& Contact currents, number of electrodes $K$
& Linear / semidefinite optimization (L1L1)
& Maximize focality or intensity
& Lead-field electric field model \\

\hline
\multicolumn{5}{l}{\textbf{Model-guided and clinical programming frameworks}}\\
\hline

\cite{frankemolle2010computational_dbs}
& Contact selection, amplitudes
& Computational model-based programming
& Improve clinical response
& Patient-specific stimulation model \\

\cite{pourfar2015guide}
& Contact, amplitude
& Model-based programming
& Clinical target selection
& Patient-specific VTA model \\

\cite{heldman2016computer_guided_dbs}
& Contact, amplitude
& Computer-guided parameter search
& Improve motor outcome
& Wearable motor-response metric \\

\cite{roediger2022stimfit}
& Contact, amplitude
& Data-driven optimization
& Symptom-response targeting
& Data-driven symptom model \\

\cite{malekmohammadi2022illumina3d}
& Contact configuration, amplitudes
& Image-guided parameter search
& Maximize target engagement
& Neuroimaging-based target model \\

\hline
\end{tabular}

\end{table*}

==> tables/Table_DBS_studies.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{p{4cm} p{3cm} p{3cm} p{3cm} p{4cm}}
\hline
\textbf{Study} & \textbf{Optimization Variables} & \textbf{Method} & \textbf{Objective Function} & \textbf{Field / Activation Approximation} \\
\hline

Peña et al. (2017) \cite{pena2017pso_dbs} 
& Contact configuration, amplitudes 
& Particle swarm optimization 
& Pathway targeting 
& Pathway activation from FEM electric fields \\

Anderson et al. (2018) \cite{anderson2018dbs_programming} 
& Contact currents 
& Nonlinear optimization 
& Target activation / avoidance suppression 
& Hessian-based activation surrogate \\

Cubo et al. (2019) \cite{cubo2019dbs_optimization} 
& Contact amplitudes 
& Constrained optimization 
& Maximize target VTA 
& VTA from electric-field thresholds \\

Galaz Prieto et al. (2022) \cite{galaz2022l1l1} 
& Contact currents, number of electrodes $K$ 
& Linear / semidefinite optimization (L1L1) 
& Maximize focality or intensity 
& Electric field / current density from lead field \\

\hline
\end{tabular}
\caption{Comparison of optimization frameworks for determining DBS electrode configurations or stimulation patterns.}
\end{table}

==> tables/Table_Medtronic.tex <==
\begin{table}[ht!]
\begin{normalsize}
\centering
\caption{Performance of the algorithm-optimized 8- and 40-contact probes on bipolar and multipolar configurations calculated using reciprocity-based principle and L1-norm fitting L1-norm Regularized (L1L1) methods, respectively, setting nuisance threshold values ranging $\varepsilon = \{-10 : 0\}$ and with range $\varepsilon = \{-160 : 0\}$ dB (decibels); target dipolar current alignment is set either {\em Parallel} (Vec 1) or {\em Perpendicular} (Vec 2) w.r.t the lead; evaluation criteria are given using {\em Focused} ($\Gamma$) and {\em Nuisance} ($\Xi$) current densities, and {\em Field ratio} ($\Theta$) over a noiseless lead field in comparison with a SNR.}
\renewcommand{\arraystretch}{1.25}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|lc|c|cccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Probe (1)\\ 8-contact\end{tabular}}} & \textbf{Bipolar} & \multicolumn{4}{c|}{\textbf{Multipolar}}                                                                                                                                                                                                                                                                                                                 \\ \cline{3-7} 
\multicolumn{2}{|c|}{}                                                                               & Reciprocity      & \multicolumn{2}{c|}{\textit{-10dB}}                                                                                                                                                   & \multicolumn{2}{c|}{\textit{-160dB}}                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{\textbf{Values}}                              & \textbf{Vec}                    & \textbf{-}       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Lead Field\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}SNR\\ Lead Field\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Lead Field\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}SNR\\ Lead Field\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Focused}}                     & 1                               & 2.820            & \multicolumn{1}{c|}{2.265}                                                                   & \multicolumn{1}{c|}{2.272}                                                             & \multicolumn{1}{c|}{2.419}                                                                   & 2.269                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 2.874            & \multicolumn{1}{c|}{2.283}                                                                   & \multicolumn{1}{c|}{2.337}                                                             & \multicolumn{1}{c|}{3.043}                                                                   & 2.345                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Nuisance}}                    & 1                               & 0.813            & \multicolumn{1}{c|}{0.101}                                                                   & \multicolumn{1}{c|}{0.118}                                                             & \multicolumn{1}{c|}{0.044}                                                                   & 0.151                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 0.813            & \multicolumn{1}{c|}{0.168}                                                                   & \multicolumn{1}{c|}{0.240}                                                             & \multicolumn{1}{c|}{0.072}                                                                   & 0.242                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Ratio}}                       & 1                               & 3.469            & \multicolumn{1}{c|}{13.075}                                                                  & \multicolumn{1}{c|}{5.482}                                                             & \multicolumn{1}{c|}{21.527}                                                                  & 5.561                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 3.535            & \multicolumn{1}{c|}{13.184}                                                                  & \multicolumn{1}{c|}{7.223}                                                             & \multicolumn{1}{c|}{27.074}                                                                  & 7.488                                                             \\ \hline
\end{tabular}%
}
%%%%%%%%%%%%%
\vskip0.5cm
%%%%%%%%%%%%%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|lc+c|cccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Probe (2)\\ 40-contact\end{tabular}}} & \textbf{Bipolar} & \multicolumn{4}{c|}{\textbf{Multipolar}}                                                                                                                                                                                                                                                                                                                 \\ \cline{3-7} 
\multicolumn{2}{|c|}{}                                                                               & Reciprocity      & \multicolumn{2}{c|}{\textit{-10dB}}                                                                                                                                                   & \multicolumn{2}{c|}{\textit{-160dB}}                                                                                                                             \\ \hline 
\thickhline
\multicolumn{1}{|l|}{\textbf{Values}}                              & \textbf{Vec}                    & \textbf{-}       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Lead Field\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}SNR\\ Lead Field\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Lead Field\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}SNR\\ Lead Field\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Focused}}                     & 1                               & 3.850            & \multicolumn{1}{c|}{2.018}                                                                   & \multicolumn{1}{c|}{2.236}                                                             & \multicolumn{1}{c|}{2.195}                                                                   & 1.737                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 3.850            & \multicolumn{1}{c|}{3.369}                                                                   & \multicolumn{1}{c|}{2.230}                                                             & \multicolumn{1}{c|}{2.235}                                                                   & 2.287                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Nuisance}}                    & 1                               & 0.741            & \multicolumn{1}{c|}{0.107}                                                                   & \multicolumn{1}{c|}{0.172}                                                             & \multicolumn{1}{c|}{0.003}                                                                   & 0.203                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 0.741            & \multicolumn{1}{c|}{0.261}                                                                   & \multicolumn{1}{c|}{0.199}                                                             & \multicolumn{1}{c|}{0.003}                                                                   & 0.160                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Ratio}}                       & 1                               & 5.195            & \multicolumn{1}{c|}{9.165}                                                                   & \multicolumn{1}{c|}{8.491}                                                             & \multicolumn{1}{c|}{526.440}                                                                 & 7.564                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & 2                               & 5.195            & \multicolumn{1}{c|}{10.965}                                                                  & \multicolumn{1}{c|}{8.469}                                                             & \multicolumn{1}{c|}{536.050}                                                                 & 9.959                                                             \\ \hline
\end{tabular}%
}
\end{normalsize}
\label{tab:Medtronic}
\end{table}

==> tables/Table_MultiComparment.tex <==
\begin{table}
\centering
\caption{The head model described was segmented utilizing the FreeSurfer software suite \cite{fischl2012freesurfer}, complemented by the segmentation interface from FieldTrip \cite{oostenveld2011fieldtrip} and SPM12 \cite{ashburner2014spm12} for the development of volumetric compartments. The assignment of piecewise constant electrical conductivity values follows the methodology proposed in \cite{dannhauer2011modeling}, which aligns the electrical conductivity characteristics of the subcortical nuclei with those of gray matter, as detailed in \cite{rezaei2021reconstructing}.
}
\begin{footnotesize}
\begin{tabular}{clccr}
\hline
 &         & \textbf{Nodes}         & \textbf{Triangles}          & \textbf{Conductivity}            \\
\textbf{ID} & \textbf{Compartment} &(\#) & (\#) & (S/m) \\
\hline
1  & Skin               & 8277          & 16550              & 0.33                    \\
2  & Skull              & 7621          & 15238              & 0.0064                  \\
3  & CSF                & 4554          & 9104               & 1.79                    \\
4  & GM                 & 17967         & 35922              & 0.33                    \\
5  & WM                 & 15238         & 30464              & 0.14                    \\
6  & Cerebellum GM      & 2870          & 5968               & 0.33                    \\
7  & Cerebellum WM      & 1081          & 2212               & 0.14                    \\
8  & Brainstem          & 381           & 760                & 0.33                    \\
9  & Cingulate cortex   & 182           & 342                & 0.14                    \\
10 & VDC                & 401           & 844                & 0.33                    \\
11 & Amygdala           & 171           & 330                & 0.33                    \\
12 & Thalamus           & 485           & 970                & 0.33                    \\
13 & Caudate            & 345           & 678                & 0.33                    \\
14 & Accumbens          & 72            & 136                & 0.33                    \\
15 & Putamen            & 402           & 800                & 0.33                    \\
16 & Hippocampus        & 465           & 918                & 0.33                    \\
17 & Pallidum           & 214           & 416                & 0.33                    \\
18 & Ventricle          & 651           & 1310               & 0.33                    \\
\hline
\end{tabular}
\begin{flushleft}
Abbreviations: CSF, cerebrospinal fluid; GM, Gray matter; WM, white matter; VDC, ventral diencephalon.
\end{flushleft}
\end{footnotesize}
\label{tab:segmentation}
\end{table}

==> tables/Table_Together.tex <==
\begin{table}[ht!]
\begin{footnotesize}
\centering
\caption{Performance summary of the algorithm-derived 8-contact and 40-contact deep brain stimulation (DBS) directional leads with bipolar configurations through reciprocity principle \cite{FERNANDEZCORAZZA2020116403}, and multipolar configurations using L1-norm fitting L1-norm Regularized (L1L1) method \cite{galazprieto_2022_L1vsL2, galazprieto_2024_lattice} with nuisance threshold values ranging $\varepsilon = \{-10 : 0\}$ and $\varepsilon = \{-160 : 0\}$ dB (decibels); target dipolar current alignment is set either {\em Parallel} (Vec 1) or {\em Perpendicular} (Vec 2) w.r.t the lead; evaluation criteria are given using {\em Focus} ($\Gamma$) and {\em Nuisance} ($\Xi$) current densities, and {\em Field ratio} ($\Theta$) over a noiseless lead field (LF) matrix in comparison with an equivalent version of the model with an {\em a priori} peak signal-to-noise (PSNR).}
\label{Tab:Together}
\renewcommand{\arraystretch}{1.25}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll+c|cccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} 8-contacts\end{tabular}}} & \textbf{Bipolar} & \multicolumn{4}{c|}{\textbf{Multipolar}}                                                                                                                                                                                                                                                                                                                 \\ \cline{3-7} 
\multicolumn{2}{|c|}{}                                                                               & \textit{RP}      & \multicolumn{2}{c|}{\textit{$\varepsilon = \{-10 : 0\}$}}                                                                                                                                                   & \multicolumn{2}{c|}{\textit{$\varepsilon = \{-160 : 0\}$}}                                                                                                                             \\ \hline
\thickhline
\multicolumn{1}{|l|}{\textbf{DV}}                              & \textbf{Orientation}                    & \textbf{-}       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}No \\ Noise \end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PSNR\\ 40 dB\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}No \\ Noise \end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}PSNR\\ 40 dB\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{$\Gamma$}}                     & Parallel                              & 2.820            & \multicolumn{1}{c|}{2.265}                                                                   & \multicolumn{1}{c|}{2.272}                                                             & \multicolumn{1}{c|}{2.419}                                                                   & 2.269                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                               & 2.874            & \multicolumn{1}{c|}{2.283}                                                                   & \multicolumn{1}{c|}{2.337}                                                             & \multicolumn{1}{c|}{3.043}                                                                   & 2.345                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{$\Xi$}}                    & Parallel                              & 0.813            & \multicolumn{1}{c|}{0.101}                                                                   & \multicolumn{1}{c|}{0.118}                                                             & \multicolumn{1}{c|}{0.044}                                                                   & 0.151                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                             & 0.813            & \multicolumn{1}{c|}{0.168}                                                                   & \multicolumn{1}{c|}{0.240}                                                             & \multicolumn{1}{c|}{0.072}                                                                   & 0.242                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{$\Theta$}}                       & Parallel                              & 3.469            & \multicolumn{1}{c|}{13.075}                                                                  & \multicolumn{1}{c|}{5.482}                                                             & \multicolumn{1}{c|}{21.527}                                                                  & 5.561                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                               & 3.535            & \multicolumn{1}{c|}{13.184}                                                                  & \multicolumn{1}{c|}{7.223}                                                             & \multicolumn{1}{c|}{27.074}                                                                  & 7.488                                                             \\ \hline
\end{tabular}%
}
%%%%%%%%%%%%%
\vskip0.5cm
%%%%%%%%%%%%%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|lc+c|cccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}40-contacts\end{tabular}}} & \textbf{Bipolar} & \multicolumn{4}{c|}{\textbf{Multipolar}}                                                                                                                                                                                                                                                                                                                 \\ \cline{3-7} 
\multicolumn{2}{|c|}{}                                                                               & \textit{RP}      & \multicolumn{2}{c|}{\textit{$\varepsilon = \{-10 : 0\}$}}                                                                                                                                                   & \multicolumn{2}{c|}{\textit{$\varepsilon = \{-160 : 0\}$}}                                                                                                                             \\ \hline 
\thickhline
\multicolumn{1}{|l|}{\textbf{DV}}                              & \textbf{Orientation}                    & \textbf{-}       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}No \\ Noise \end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PSNR\\ 40 dB\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}No \\ Noise\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}PSNR\\ 40 dB\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Focus}}                     & Parallel                               & 3.850            & \multicolumn{1}{c|}{2.018}                                                                   & \multicolumn{1}{c|}{2.236}                                                             & \multicolumn{1}{c|}{2.195}                                                                   & 1.737                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                              & 3.850            & \multicolumn{1}{c|}{3.369}                                                                   & \multicolumn{1}{c|}{2.230}                                                             & \multicolumn{1}{c|}{2.235}                                                                   & 2.287                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Nuisance}}                    & Parallel                               & 0.741            & \multicolumn{1}{c|}{0.107}                                                                   & \multicolumn{1}{c|}{0.172}                                                             & \multicolumn{1}{c|}{0.003}                                                                   & 0.203                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                               & 0.741            & \multicolumn{1}{c|}{0.261}                                                                   & \multicolumn{1}{c|}{0.199}                                                             & \multicolumn{1}{c|}{0.003}                                                                   & 0.160                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Ratio}}                       & Parallel                               & 5.195            & \multicolumn{1}{c|}{9.165}                                                                   & \multicolumn{1}{c|}{8.491}                                                             & \multicolumn{1}{c|}{526.440}                                                                 & 7.564                                                             \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                                             & Perpendicular                              & 5.195            & \multicolumn{1}{c|}{10.965}                                                                  & \multicolumn{1}{c|}{8.469}                                                             & \multicolumn{1}{c|}{536.050}                                                                 & 9.959                                                             \\ \hline
\end{tabular}%
}
\end{footnotesize}
\end{table}

==> tables/Table_Uncertainty_DBS.tex <==
\begin{table*}[t]
\centering
\caption{Uncertainty quantification studies relevant to deep brain stimulation (DBS) field modeling and electrode localization.}
\label{tab:uq_dbs}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{p{3.3cm} p{2.4cm} p{3.3cm} p{2.2cm} p{5.6cm}}
\hline
\textbf{Study} & \textbf{Lesion} & \textbf{Affected tissue / compartment} & \textbf{\# electrodes} & \textbf{Electrical characteristics / uncertainty modeled} \\
\hline
Butson \& McIntyre (2006) & None (DBS therapy context) & Electrode geometry; tissue surrounding electrode (VTA dependence) & 4 contacts & Sensitivity of VTA to electrode design and stimulation parameters; provides baseline model-structure uncertainty and field-shape dependence on electrode geometry. \\
Chaturvedi et al. (2010) & None (patient-specific DBS) & Electrode--tissue interface, encapsulation layer, tissue anisotropy/inhomogeneity & 4 contacts & Compares model complexities (incl.\ electrode interface and encapsulation) and shows prediction differences; captures uncertainty due to omitted physics/compartments. \\
Schmidt et al. (2012) & None (DBS FEM with UQ) & GM/WM/CSF conductivities; encapsulation layer conductivity & 4 contacts (DBS electrode model) & Explicit conductivity uncertainty quantification in heterogeneous DBS FEM using polynomial chaos / non-intrusive projection; produces probabilistic field/VTA variability due to parameter uncertainty. \\
Sitz et al. (2017) & None (phantom study) & Lead orientation reconstruction (directional lead markers) & N/A (directional lead; contact count not required for orientation) & Imaging-based uncertainty in directional lead orientation estimation (CT vs x-ray); quantifies orientation error that propagates into current steering predictions. \\
Lasica et al. (2025) & Parkinson's disease cohort (localization study) & Post-operative electrode contact localization; VTA overlap variability & N/A (DBS lead type montage-dependent) & Quantifies electrode reconstruction uncertainty across software and raters (mm-scale contact localization variability; VTA Dice overlap variability). \\
\hline
\end{tabular}
\end{table*}

==> tables/Table_Uncertainty_tES.tex <==
\begin{table*}[t]
\centering
\caption{Uncertainty quantification studies relevant to transcranial electrical stimulation (tES) forward modeling.}
\label{tab:uq_tes}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{p{3.3cm} p{2.4cm} p{3.3cm} p{2.2cm} p{5.6cm}}
\hline
\textbf{Study} & \textbf{Lesion} & \textbf{Affected tissue / compartment} & \textbf{\# electrodes} & \textbf{Electrical characteristics / uncertainty modeled} \\
\hline
Datta et al. (2010) & Skull defect / skull plate & Skull defect region, skull, cortex (current shunting at defect boundary) & 2 (tDCS pads) & Sensitivity of predicted fields to altered skull integrity and defect/plate conductivity (model-parameter uncertainty impacting field magnitude and distribution). \\
Opitz et al. (2015) & None (healthy) & Skull layers, CSF, gray/white matter (incl.\ anisotropy) & 2 (tDCS pads) & Sensitivity of field distribution to anatomical features (skull/CSF geometry, anisotropy); highlights model-parameter/segmentation-driven variability in induced fields. \\
Saturnino et al. (2019) & None (method paper; examples in NIBS) & Tissue conductivities (whole-head compartments as uncertain parameters) & N/A (method; montage-dependent) & Formal conductivity uncertainty propagation and sensitivity analysis (generalized polynomial chaos) quantifying reliability of field estimates under conductivity variability. \\
McCann et al. (2019) & None (meta-analysis) & Head tissue conductivities (multiple tissues) & N/A & Meta-analysis quantifying variability in reported conductivity values (population/literature-driven parameter uncertainty bounds used in forward models). \\
Huang et al. (2016) & None (standardized head model) & Whole-head compartments; electrode placement/model standardization & N/A (model supports tES targeting) & Standardized FEM head model assessing localization/targeting errors; relevant to uncertainty from anatomical standardization and electrode representation/placement assumptions. \\
Vorwerk et al. (2014) & None (guideline paper) & Head compartments, skull modeling, CSF, anisotropy, discretization choices & N/A & Quantifies impact of modeling choices (compartment inclusion, conductivity assumptions, discretization) on forward solution accuracy; used as methodological uncertainty reference. \\
\hline
\end{tabular}
\end{table*}

==> tables/Table_hyperparameters.tex <==
\begin{table}
    \centering
    \begin{footnotesize}
    \caption{Summary of the proposed optimization methods. RP provides a bipolar reciprocal of the target, whereas L1L1 and TLS perform an extensive metaheuristic search. L1L1 method is subdivided into L1L1(A) and L1L1(B) according to two alternative {\em a priori} assumptions for the feasible $\varepsilon$ threshold range: [-160, 0]~dB and [-10, 0]~dB, respectively. The regularization and L2-norm weighting parameter ranges are adopted from \cite{galazprieto_2022_L1vsL2}. CPU time refers to the computation time needed to evaluate a single optimizer with fixed hyperparameters for the HR-LF using the 40-contact lead.}
    \label{tab:hyperparameters}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{llllr}
    \toprule
    \textbf{Optimization} & \textbf{Search} &  {\bf Tuning Range } & {\bf Role} & {\bf Time} \\ 
    {\bf Method} & {\bf Type} &  {\bf (dB)} &  & {\bf (s)} \\ 
    \midrule
    {RP} & Reciprocal & -- & -- & 5.7E-03 \\ 
    {{L1L1(A)}} & Metaheuristic & $\alpha \in [-100, -30]$  & Regularization & \multirow{2}{*}{6.0} \\ 
    & & $\varepsilon \in [-160, 0]$ & Threshold &  \\ 
    {{L1L1(B)}} & Metaheuristic & $\alpha \in [-100, -30]$ & Regularization & \multirow{2}{*}{3.7} \\ 
    & & $\varepsilon \in [-10, 0]$ & Threshold &  \\ 
    {TLS} & Metaheuristic & $\gamma \in [-200, -110]$ & Regularization & \multirow{2}{*}{5.0E-02} \\ 
    & & $\beta \in [-50, 40]$ & Weight &  \\ 
    \bottomrule
    \end{tabular}}
    \end{footnotesize}
\end{table}

==> workbench.tex <==
    \begin{minipage}{16.5cm}
        \begin{tabular}{|cc|cc|cc|cc|}
        %\hline
        \includegraphics[width=0.50cm, height = 5cm]{Figure_Contacts/AB_HR_RP_DBSlead.png} &
        \begin{minipage}[b]{2.85cm}
            \centering
            \vskip0.2cm
            RP \\
            \includegraphics[width=2.85cm, height=2.25cm]{Figure_Contacts/AB_HR_RP_barplot.png} \\ \vskip0.2cm
            \includegraphics[width=1.85cm, height=2.25cm]{Figure_Contacts/AB_HR_RP_electrodes.png} \vskip0.2cm
        \end{minipage} &
        \includegraphics[width=0.50cm, height = 5cm]{Figure_Contacts/AB_HR_L1L1eps160_DBSlead.png} &
        \begin{minipage}[b]{2.85cm}
            \centering
            \vskip0.2cm
            L1L1(A) \\
            \includegraphics[width=2.85cm, height=2.25cm]{Figure_Contacts/AB_HR_L1L1eps160_barplot.png} \\ \vskip0.2cm
            \includegraphics[width=2.10cm, height=2.25cm]{Figure_Contacts/AB_HR_L1L1eps160_electrodes.png} \vskip0.2cm 
        \end{minipage} &
        \includegraphics[width=0.50cm, height = 5cm]{Figure_Contacts/AB_HR_L1L1eps10_DBSlead.png} &
        \begin{minipage}[b]{2.85cm}
            \centering
            \vskip0.2cm
            L1L1(B) \\
            \includegraphics[width=2.85cm, height=2.25cm]{Figure_Contacts/AB_HR_L1L1eps10_barplot.png} \\ \vskip0.2cm
            \includegraphics[width=2.35cm, height=2.25cm]{Figure_Contacts/AB_HR_L1L1eps10_electrodes.png} \vskip0.2cm
        \end{minipage} &
        \includegraphics[width=0.50cm, height = 5cm]{Figure_Contacts/AB_HR_TLS_DBSlead.png} &
        \begin{minipage}[b]{2.85cm}
            \centering
            \vskip0.2cm
            TLS \\
            \includegraphics[width=2.85cm, height=2.25cm]{Figure_Contacts/AB_HR_TLS_barplot.png} \\ \vskip0.2cm
            \includegraphics[width=2.50cm, height=2.25cm]{Figure_Contacts/AB_HR_TLS_electrodes.png} \vskip0.2cm
        \end{minipage} \\
        %\hline
        \end{tabular}
    \end{minipage}
